Aligning Large Language Models for Controllable Recommendations

Inspired by the exceptional general intelligence of Large Language Models (LLMs), researchers have begun to explore their application in pioneering the next generation of recommender systems - systems that are conversational, explainable, and controllable. However, existing literature primarily concentrates on integrating domain-specific knowledge into LLMs to enhance accuracy, often neglecting the ability to follow instructions. To address this gap, we initially introduce a collection of supervised learning tasks, augmented with labels derived from a conventional recommender model, aimed at explicitly improving LLMs' proficiency in adhering to recommendation-specific instructions. Subsequently, we develop a reinforcement learning-based alignment procedure to further strengthen LLMs' aptitude in responding to users' intentions and mitigating formatting errors. Through extensive experiments on two real-world datasets, our method markedly advances the capability of LLMs to comply with instructions within recommender systems, while sustaining a high level of accuracy performance.

==> sections/A1_sensitivity_analysis.tex <==
\subsection{Sensitivity analysis}
\label{app:sensitivity_analysis}

% 我们对RL阶段中的，用于衡量用户偏好与意图的$\alpha$超参数进行了敏感度分析。在Steam数据集中，我们分别测试了$\alpha$ in [0.2,0.5,0.8]。然后我们统计了它们在$I_2^{CP\leq20\%}$，$I_2^{CP\approx30\%}$，$I_2^{CP\geq30\%}$这三类指令上的推荐准确率和控制准确率，$Acc_{rec}$是三类指令的NDCG@10指标的平均值，$Acc_{ctl}$是三类指令CPA指标的平均值。\autoref{fig:sensitive_analysis}结果显示，$\alpha=0.5$是一个较优的选择。

We conducted a sensitivity analysis on the $\alpha$ hyperparameter used to measure user preferences and intentions during the Reinforcement Learning (RL) stage. In the Steam dataset, we tested $\alpha$ in the range of [0.2, 0.35, 0.5, 0.65, 0.8]. 
Subsequently, we calculated their recommendation accuracy and control accuracy on three types of instructions: $I_2^{CP\leq20\%}$, $I_2^{CP\approx30\%}$, and $I_2^{CP\geq30\%}$. Here, $Acc_{rec}$ represents the average NDCG@10 metric for these three types of instructions, and $Acc_{ctl}$ represents the average CPA metric for the same instructions. The results shown in \autoref{fig:sensitive_analysis} indicate that 0.35 or 0.5 is a preferable choice to balance $Acc_{rec}$ and $Acc_{ctl}$.
\begin{figure}[h]
\setlength{\abovecaptionskip}{0.1cm}
\centering
\includegraphics[width=1.0\linewidth]{figures/sensitive_analysis.pdf}
\caption{Sensitive analysis in different $\alpha$.}
\label{fig:sensitive_analysis}
\vspace{-0.3cm}
\end{figure}


==> sections/A2_case_study.tex <==
\subsection{Additional case study}
\label{app:additional_case_study}


==> tables/1_model_description.tex <==
\begin{table}[t]
\setlength{\abovecaptionskip}{0.1cm}
\resizebox{0.47\textwidth}{1.2cm}{
\begin{tabular}{l|cccc}
\toprule
% \cmidrule(lr){2-3}\cmidrule(lr){4-5}
Model Name & $\mathrm{SL_{I_{\{0\}}}}$ & $\mathrm{SL_{I_{\{1,2,3,4\}}}}$ & $\mathrm{RL}$ & $\mathrm{RW_{item}}$ \\
\midrule
$\mathrm{Ours_{v1}}$  & \Checkmark & \XSolidBrush & \XSolidBrush & \XSolidBrush \\
$\mathrm{Ours_{v2}}$  & \Checkmark & \Checkmark & \XSolidBrush & \XSolidBrush \\
$\mathrm{Ours_{v3}}$  & \Checkmark & \Checkmark & \Checkmark & \XSolidBrush \\
$\mathrm{Ours_{v3}}$  & \Checkmark & \Checkmark & \Checkmark & \Checkmark \\
\bottomrule
\end{tabular}
}
\caption{Model description}
\label{tab:ModelDescription}
% \vspace{-0.2cm}
\end{table}

